Fast-Grasp'D: Dexterous Multi-finger Grasp Generation Through Differentiable Simulation

Multi-finger grasping relies on high quality training data, which is hard to obtain: human data is hard to transfer and synthetic data relies on simplifying assumptions that reduce grasp quality. By making grasp simulation differentiable, and contact dynamics amenable to gradient-based optimization, we accelerate the search for high-quality grasps with fewer limiting assumptions. We present Grasp'D-1M: a large-scale dataset for multi-finger robotic grasping, synthesized with Fast- Grasp'D, a novel differentiable grasping simulator. Grasp'D- 1M contains one million training examples for three robotic hands (three, four and five-fingered), each with multimodal visual inputs (RGB+depth+segmentation, available in mono and stereo). Grasp synthesis with Fast-Grasp'D is 10x faster than GraspIt! and 20x faster than the prior Grasp'D differentiable simulator. Generated grasps are more stable and contact-rich than GraspIt! grasps, regardless of the distance threshold used for contact generation. We validate the usefulness of our dataset by retraining an existing vision-based grasping pipeline on Grasp'D-1M, and showing a dramatic increase in model performance, predicting grasps with 30% more contact, a 33% higher epsilon metric, and 35% lower simulated displacement. Additional details at https://dexgrasp.github.io.

==> 00-format-and-definitions.tex <==
\usepackage{graphicx}
\usepackage{epsfig}

\usepackage{subcaption}
\usepackage{float}
\usepackage[font=small]{caption}

\usepackage{multicol}

\usepackage{bm}                          % Make bold, italic math symbols
\usepackage{mathtools}
\usepackage{amsmath, amssymb, amscd}
\usepackage{bm}
\usepackage{wasysym} %special symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{mdwmath}
\usepackage{eqparbox} %equations
\usepackage{array} %equations
\usepackage{nicefrac}

\usepackage{array} %for table entries to be in center of cell
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs}   % Publication quality tables

\usepackage{listings}
\usepackage{nameref}
\usepackage{paralist}
\usepackage{xspace}
\usepackage{setspace}

\usepackage{graphicx}
\usepackage{subcaption}
\usepackage[font=small]{caption}

\usepackage{float}
\usepackage{lscape}

\usepackage{booktabs}
\usepackage{multirow}

\usepackage{paralist}
%\usepackage{enumitem}

\usepackage{bm}
\usepackage{epsfig}
\usepackage{mathtools}

%\usepackage{color,colortbl}
\usepackage{siunitx}

\usepackage[table,xcdraw]{xcolor}

\makeatletter
\let\NAT@parse\undefined
\makeatother
\usepackage[numbers,sort]{natbib}


\renewcommand {\vec}[1]{\mathbf{#1}}
\newcommand {\pi}{\vec{p_i}}
\newcommand {\pstar}{\vec{p^*}}
\newcommand {\prhostar}{\vec{p_rho^*}}
\newcommand {\qq}{\vec{q}}
\newcommand {\dqq}{\dot{\vec{q}}}
\newcommand {\ddqq}{\ddot{\vec{q}}}
\newcommand {\duu}{\dot{\vec{u}}}
\newcommand {\dduu}{\ddot{\vec{u}}}
\newcommand {\uu}{\vec{u}}
\newcommand {\HH}{\textbf{H}}
\newcommand {\MM}{\textbf{M}}
\newcommand {\fc}{\vec{f}_\textrm{c}}
\newcommand {\funfc}{f_\textrm{c}}
\newcommand {\fe}{\vec{f}_\textrm{ext}}
\newcommand {\Xh}{\textbf{X}_\textrm{h}}
\newcommand {\xh}{\vec{x}}
\newcommand {\x}{\vec{x}}
\newcommand {\R}{\vec{R}}
\newcommand {\piii}{\vec{p_i}}
\newcommand {\fn}{\vec{f}_n}
\newcommand {\ft}{\vec{f}_t}
\newcommand {\kn}{k_n}
\newcommand {\kf}{k_f}
\newcommand {\vt}{\vec{v}_t}
\newcommand {\xlocal}{\vec{x}_\textrm{local}}
\newcommand {\pclosest}{\vec{p}_\textrm{closest}}
\newcommand {\pclosestp}{\vec{p}_\textrm{phong}}
\newcommand {\xclamp}{\vec{x}_\textrm{clamp}}
\newcommand {\ffn}{f_n}
\newcommand {\fft}{f_t}
\newcommand\norm[1]{\Vert#1\Vert}
\newcommand {\qh}{\qq_{\textrm{h}}}
\newcommand {\qobj}{\vec{q}_{\textrm{o}}}
\newcommand {\qhand}{\vec{q}_{\textrm{hand}}}
\newcommand {\dqobj}{\dot{\vec{q}}_\textrm{o}}
\newcommand {\fd}{\widehat{\vec{f}}_\textrm{c}}
\newcommand {\Fd}{\vec{F}_\textrm{desired}}
\newcommand {\Fc}{\vec{F}_\textrm{actual}}
\newcommand {\Ltask}{\mathcal{L}_\textrm{task}}
\newcommand {\Lphysics}{\mathcal{L}_\textrm{phys}}
\newcommand {\uobj}{\uu_\textrm{obj}}
\newcommand {\duobj}{\dot{\vec{u}}_\textrm{o}}
\newcommand {\uh}{\uu_\textrm{h}}
\newcommand {\duh}{\dot{\vec{u}}_\textrm{h}}
\newcommand {\Lqrange}{\mathcal{L}_\textrm{range}}
\newcommand {\Lqlimit}{\mathcal{L}_\textrm{limit}}
\newcommand {\Linter}{\mathcal{L}_\textrm{inter}}
\newcommand {\finter}{\vec{f}_\textrm{link}}
\newcommand {\phong}{\phi_{\textrm{phong}}}

\definecolor{Lightapricot}{rgb}{0.99,0.84,0.69}

\makeatletter
\newcolumntype{B}[3]{>{\boldmath\DC@{#1}{#2}{#3}}c<{\DC@end}}
\makeatother


==> 00-paper-todos.tex <==
time: 5:50pm

----
text
----

- methods
- experimental setup 
- results paragraphs for dataset comparison and ddgc

----
figures
----
google slides link:

- teaser figure 3x3 block with 3 hands. 
(expected in 30 mins)
- fig2: cherry pick good examples. 
(expected time 30 mins)
- fig 3 qualitative figure
(expected time 1 hour)
-fig 4 - plot thresh contact vs metrics!
fig 5: Dylan!


----
numbers/tables
----



----
website
----
- heatmap interactive 3D


----
Long term wishlist
----
- add 2 finger robotique hand 
- add mano hand grasps -- why ? -- can be useful for vision people 
- is two-finger grasping improved if we use Fast-Grsp'D vs current methods?
- large scale real-world evaluation of generated grasps
    -  grasp, pick, drop, grasp. ....
    - grasp, pick, inhand change grasp, ....
    - grasp, pick, use env contact to arrive at new grasp
    
- can we model slip well? say oily/greasy object -- use env contact to stabilize

- is there a memory limit at 32? can we create a plot of scaling perf with batch size
